The Expressive Power of Transformers with Chain of Thought

Recent theoretical work has identified surprisingly simple reasoning problems, such as checking if two nodes in a graph are connected or simulating finite-state machines, that are provably unsolvable by standard transformers that answer immediately after reading their input. However, in practice, transformers' reasoning can be improved by allowing them to use a "chain of thought" or "scratchpad", i.e., generate and condition on a sequence of intermediate tokens before answering. Motivated by this, we ask: Does such intermediate generation fundamentally extend the computational power of a decoder-only transformer? We show that the answer is yes, but the amount of increase depends crucially on the amount of intermediate generation. For instance, we find that transformer decoders with a logarithmic number of decoding steps (w.r.t. the input length) push the limits of standard transformers only slightly, while a linear number of decoding steps, assuming projected pre-norm (a slight generalization of standard pre-norm), adds a clear new ability (under standard complexity conjectures): recognizing all regular languages. Our results also imply that linear steps keep transformer decoders within context-sensitive languages, and polynomial steps with generalized pre-norm make them recognize exactly the class of polynomial-time solvable problems -- the first exact characterization of a type of transformers in terms of standard complexity classes. Together, this provides a nuanced framework for understanding how the length of a transformer's chain of thought or scratchpad impacts its reasoning power.

==> neurips-workshop/2024-rightmost-hash/general-tm.tex <==
\change{The relatively simple proof of \Cref{thm:lower-bound} relies on the slight architectural extension of multi-pre-norm. Without multi-pre-norm, it is still possible to simulate a Turing machine with linear overhead, though the overhead factor increases and the construction becomes more complicated:}

\begin{restatable}[Proof in \Cref{sec:general-tm-proof}]{theorem}{generaltm} \label{thm:lower-bound-general}
    Let $M$ be a Turing machine that, on input length $n$, runs for at most $t(n)$ steps (at most polynomial).
    % Let $\pi$ be a positional encoding scheme that allows separating the first token.
    % Then 
    For any start-separable positional encoding,
    there is a decoder-only saturated transformer that, on input $x$, computes $M(x)$ with $6 t(n) + 3 \abs{M(x)}$ decoding steps.
\end{restatable}

\change{The construction with multi-pre-norm is simpler and requires less overhead, which may suggest exploring this extension to transformers in practice.}

% \ashish{see comments earlier about moving these caveats and architecture suggestions to earlier} \will{moved up}
% As mentioned earlier, in contrast to \citet{perez2021attention}, \Cref{thm:lower-bound} does not assume nonstandard positional encodings. However, it does assume causally masked attention cannot attend to the current token. Interestingly, two minor architectural changes to the transformer could simplify details of the construction. First, having a linear layer before layer-norm would avoid the need for $\phi_z$ since it would be straightforward to preserve information in the residual connection that is not used in layer-norm computation. Second, having multiple projections of the state with different layer-norms at the beginning of the layer simplify computing rightmost hard attention. We take this as a weak sign that architectural changes along these lines \ashish{such as (multiple) selective layer-norm? giving it a name will help} would be worth exploring.

%%%%%%%%%%%%%%%%%

\section{General Turing Machine Simulation Proof} \label{sec:general-tm-proof}

\generaltm*

\begin{proof}
    The high-level idea is similar to \Cref{thm:lower-bound} except that we will make two inefficient changes to the simulation to make the construction work without multi-pre-norm. Let $T = t(n)$ be the total number of decoding steps.
    \begin{compactenum}
        \item We left-pad the decoding steps with $3T$ no-op steps. \will{We should be able to implement this by counting as long as $t(n)$ is polynomial. Every $n$ steps, write a symbol $k_1$, then every $n$ $k_1$'s, write $k_2$, etc. Is there a cleaner way?}
        
        \item We intersperse 2 no-op steps between each step simulating a Turing machine step. This can be implemented by outputting a modular counter along with the standard output of each step.
    \end{compactenum}
    This means decoding step $i = n + 3T + 3i'$ will simulate Turing machine step $i'$. We now modify the inductive case from \Cref{thm:lower-bound} to accord with this construction.

    \underline{Inductive Case}. We describe the construction of each step $i = n + 3T + 3i'$. We first reconstruct $h^\tau_i / i$ as for \Cref{thm:lower-bound}, with the extension that no-op steps contribute a move direction of 0. Thus, $h^\tau_i / i$ represents the position on tape $\tau$ at Turing machine step $i$.

    \will{TODO: adapt input tape construction}

    Next, we show a modified construction to retrieve the contents at $h^\tau_i$ for each non-input tape $\tau$. This time, we will use a different layer for each head, each with a single layer-norm.
    W.l.o.g., finite state such as the output of each layer can be stored in the residual stream without appearing in the layer-norm hash because of the stateful extension of the hash (cf.~\Cref{sec:stateful-lnorm-hash}). This will be important for aggregating the layer outputs.

    The layer-norm hash computed at position $i$ by layer $\tau$ from the residual stream is \ashish{describe how to get rid of $n$}
    \begin{align*}
        \phi^\tau_i
        &\triangleq \phi(h^\tau_i / (i - n), 1/(i - n - 1)) = \phi(h^\tau_i, (i - n)/(i - n - 1)) \\
        &= \phi ( h^\tau_i, c_i), \quad \textrm{where} \; c_i \triangleq \frac{i - n}{i - n - 1} = \frac{3T + 3i}{3T + 3i - 1} = \frac{T + i}{T + i - 1/3}.
    \end{align*}
    We attend with query $\phi^\tau_i$, key $\phi^\tau_j$, and value $[\delta_j]_{2 + \tau}$.
    For any $j \leq i \leq T$, we have $T + j > \frac{T + i}{2}$. Thus, $c_j < c_{i/2}$. \will{check}
    The preconditions of \Cref{lem:rightmost-lnorm} are met, so attention is maximized for the largest $j < i$ such that $h^\tau_i = h^\tau_j$. The head thus retrieves $\gamma^\tau_i$: the most recent update written to tape $\tau$ at position $h^\tau_i$. \will{Is it okay that $c_t$ has $n + 3T$ in num/denom? rather than just $3t/(3t - 1)$?}

    We now have the state and layer outputs stored in the residual stream.
    Following \Cref{thm:lower-bound}, we compute $\delta_{i-n} = \delta(q_i, \gamma^0_i, \ldots, \gamma^{k + 1}_i)$ using a feedforward network and output it, completing the inductive step.

    \will{Describe how to reconstruct output}
\end{proof}

==> neurips-workshop/2024-rightmost-hash/old-junk.tex <==
\begin{proof}
    Without loss of generality, we show a construction for transformers with $1/i$ positional encodings (cf.~\Cref{lem:start-separable}).
    We will construct a transformer decoder that simulates a Turing machine in linear time: three transformer decoding steps will simulate one Turing machine step. This means the simulation will take $3t(n)$ steps, followed by an additional $3\ell(n)$ steps to reconstruct the output. The main difficulty will be constructing a distributed representation of a Turing machine tape in a sequence of transformer state vectors and showing how the transformer can both maintain this representation and correctly reconstruct the current status of the tape at the head position. The key idea to the construction will be to store ``diffs'' to the tape at each timestep and use the layer-norm hash to dynamically reconstruct the contents at the head position at every new timestep.

    We introduce a new finite vocabulary $\Delta$ and identify each element of $Q \times \Gamma^{k+1} \times \{\pm 1 \}^{k+2}$ with some $\delta \in \Delta$. A deterministic Turing machine run of length $m$ induces a \emph{diff sequence} $\delta_0, \ldots, \delta_m \in \Delta$ capturing the state entered, tokens written, and directions moved after each token.
    We work with a $3{\times}$ redundant diff sequence: $\delta_{3t}$ to $\delta_{3t + 2}$ all write the same token to three adjacent tape positions.
    \change{We show by induction over $t$ that we can output $\delta_{3t + \pi}$ at intermediate step $3t + \pi$, for $\pi \in \{0, 1, 2\}$.
    For technical reasons, we will also output the modular offset $\pi_i \in \{0, 1, 2\}$ along with $\delta_i$.


    % as well as a token $\pi_i \triangleq i \bmod 3$ at decoding steps $3t + \pi$ for $\pi \in \{0, 1, 2\}$.
    \underline{Base Case: $t = 0$.} Output $\delta_0 = \langle q_0, b^k, 1 \rangle$ at the final 3 input tokens (w.l.o.g. assume length 3 input).
    }

    \underline{Inductive Case:}
    We first use a single layer to reconstruct each $h^\tau_i$, the current position on tape $\tau$ at step $i$. For each $\tau$, a head attends uniformly over the full left context where the value at a decoding step $j$ is the move direction of $\tau$ at $j$.
    Head $\tau$ thus computes $h^\tau_i/i$.

    \change{We now describe step $i = n + 3t$, which is the main part of the construction.
    The first task is to find token $h^0_i$ of the input tape with attention. For this, at each index $i$, we define $x_i, y_i$ as
    \begin{equation*}
        \langle x_i, y_i \rangle = \begin{cases}
            \langle 1, 1/i \rangle & \textrm j \leq n \\
            \langle h^0_i/i, 1/i \rangle & \textrm{otherwise} .
        \end{cases}
    \end{equation*}
    Let $\langle \cdot \rangle$ be vector concatenation.
    We use the stateful extension of the layer-norm hash ($\hash_z$, \Cref{sec:stateful-lnorm-hash}) to propagate $q_{i-1}$ to the next layer while using the hash.
    Let $\mathbf W$ be the linear transformation defined in \Cref{lem:stateful-hash}.
    We attend with key $\langle \mathbf W \phi_z(x_i, y_i), 1 \rangle$, query $\langle \mathbf W \phi_z(x_j, y_j), \mathbbm{1}[j \leq n] \rangle$ and value $\sigma_j$. By \Cref{lem:stateful-hash}, the attention score is maximized for some $j \leq n$ such that $\phi(x_i, y_i) = \phi(x_j, y_j)$. For $i > n$ and $j \leq n$, this means $\phi_{h^0_i} = \phi_j$. By \Cref{lem:lnorm-unique}, the head retrieves $\sigma_{h^0_i}$. Columns $3t + 1$ and $3t + 2$ compute $0$ queries for this head and do not move on the tape.
    }

    % \will{For single-tape TM, no issue. For multi-tape, we can split across layers. Then keep $\delta$'s in residual connection. Use stateful hash and invoke \Cref{lem:stateful-hash} to justify that it behaves analogously to normal hash. Then call \Cref{lem:lnorm-unique} to analyze in terms of normal hash.}
    \change{Next, we use $k$ different layers to get the position $h^\tau_i$ on each non-input tape $\tau$. In addition to the stateful hash, we will use the layer-norm hash in a way that enables rightmost hard attention (\Cref{sec:rightmost-lnorm-hash}). In each layer, we first compute $\phi^\tau_i \triangleq \hash_z(h^\tau_i/i, 1/(i-1))$ at each $i$.
    % Let $\mathbf W$ be the linear transformation defined in \Cref{lem:stateful-hash}.
    % and $\langle \cdot \rangle$ denote vector concatenation.
    % We construct a head that attends with query $\langle \mathbf W \phi^\tau_i, 1 \rangle$ over keys $\langle \mathbf W \phi^\tau_j, -1/j \rangle$ and values $\delta_{h^\tau_j}$, for $j \leq i$.
    We construct a head that attends with query $\mathbf W \phi^\tau_i$ over keys $\mathbf W \phi^\tau_j$ and values $\delta_{h^\tau_j}$, for $j < i$.
    We will justify that this head attends to the rightmost $j < i$ such that $h^\tau_j = h^\tau_i$ and thus retrieves the last update to the tape position at step $i$.
    First, we apply \Cref{lem:stateful-hash} to rewrite $\mathbf W \phi^\tau_i$ as
    \begin{equation*}
        \mathbf W \phi^\tau_i = \hash(h^\tau_i/i, 1/(i-1)) .
    \end{equation*}
    Next, we can use the scale invariance of the layer-norm hash to simplify
    \begin{equation*}
        \mathbf W \phi^\tau_i = \hash(h^\tau_i, i/(i-1)) .
    \end{equation*}
    Finally, by \Cref{lem:rightmost-lnorm}, $(\mathbf W \phi^\tau_i) \cdot (\mathbf W \phi^\tau_j)$ is maximized for the greatest $j < i$ s.t. $h^\tau_j = h^\tau_i + \pi$ for some $\pi \in \{0, 1, 2\}$. By construction, the last updates at tape cells $h^\tau_{3t}$ through $h^\tau_{3t} + 2$ are the same.
    Thus, at step $3t$, the head retrieves the most recent update to the current tape cell at step $h^\tau_{3t}$, which we denote $d^\tau_i$.}

    % ========
    % OLD
    % ========
    % \will{old} \underline{Inductive Case:} We can now apply $k$ different layer-norm hashes to get $\phi^\tau_i \triangleq \hash(h^\tau_i/(n+i), 1/(n+i))$ in parallel at each $i$. By \Cref{lem:lnorm-unique}, the inner product $\phi^\tau_i \cdot \phi^\tau_j$ is maximized when $h^\tau_i$ and $h^\tau_j$ are equal. For each $\tau$ we construct a head that hard-attends with query $\langle \phi^\tau_i, 1 \rangle$ over keys $\langle \phi^\tau_j, -1/j \rangle$ and values $\delta_{h^\tau_j}$, for $j \leq i$. This returns the last update $d^\tau_i$ written to the head position at step $i$.

    We now have all the necessary inputs to compute the next Turing machine transition.
    For each $\tau \geq 0$, the second component of $d^\tau_i$ is $\gamma^\tau_i$: the current contents of cell $h^\tau_i$ of tape $\tau$. As input to column $i$ of the transformer, we have $\delta_{i - 1}$, which contains $q_{i-1}$. We now compute
    % \begin{equation*}
        $\delta_i = \delta(q_{i-1}, \gamma^0_i, \ldots \gamma^{k + 1}_i)$
    % \end{equation*}
    using a feedforward network, which is possible because this computation is simply a finite table lookup. We write out $\delta_i$ as the output of column $i = n + 3t$.

    \change{To compute the inductive step, at $3t + 1$ and $3t + 2$, we simply copy the output token from $3t$. If the original Turing machine moved right, we move $1, 1, 1$ after each step. On the other hand, if the original machine moved left, we move $1, 1, -5$ after each step. This ensures that the cell contents of $h_i$ to $h_{i + 2}$ are populated correctly and that $h_{i + 3}$ is correctly represents $3(t \pm 1)$. Finally, we update the modular counter $\pi_i$ based on $\pi_{i-1}$ using a simple table lookup.}

    To conclude, we use at most $3\abs{M(x)}$ steps to reconstruct the Turing machine output. Analogously to above, we retrieve $d^{k+1}_i$, the last update written to the current head position on the output tape, and output $\gamma^{k+1}_i$. We then write a diff $\delta_i$ that moves the head to the right. We iterate in this state until $b$ (blank) is read, at which point we halt.
    We conclude that we are able to simulate $M$ in real-time, i.e., the transformer runs one decoding step per step of $M$ followed immediately by $M$'s output.
\end{proof}

==> neurips-workshop/2024-rightmost-hash/ratio-lemmas.tex <==
\subsection{Stateful Layer-Norm Hash with Finite State} \label{sec:stateful-lnorm-hash}

We consider the setting where we would like to use the layer-norm hash on part of the hidden state $h_i$, but $h_i$ also contains some additional finite state independent of the hash key that we would like to propagate to later layers. Formally, let $x$ be the hash value at token $i$ and $z \in [0, Z]$ be the additional finite state, encoded as an integer bounded by $Z$.

\begin{definition}[$z$-stateful layer-norm hash]
    Recall that, in the original layer-norm hash, $\phi(x/i, 1/i) = \lnorm(\mathbf v)$ where $\mathbf v \triangleq \langle x/i, 1/i, -x/i, -1/i \rangle$. For the $z$-stateful hash, we instead let $\mathbf v_z$ be the ``$\mathbf v$-hot'' vector of length $4Z$ with $\mathbf v$ at indices $4z + 1$ to $4(z + 1)$ and $0$ everywhere else. Then, the \emph{$z$-stateful layer-norm hash} is $\phi_z(x/i, 1/i) \triangleq \lnorm (\mathbf v_z)$.
\end{definition}

\change{We can always compute the stateful layer-norm hash in place of the standard layer-norm hash as follows.
Imagine $x, y$ are outputs of attention heads or constants, and the finite state $z$ is encoded as a one-hot vector $z_1, \ldots, z_Z$. We then map $x, y$ to a ``one-hot'' vector $\mathbf v = \langle 0, \ldots, x, y, -x, -y, \ldots, 0 \rangle$, where $x, y$ starts at $4z + 1$, via a simple linear transformation (essentially, table lookup) \will{Is this valid?}.
Then, the next layer computes
\begin{equation*}
    \lnorm(\mathbf v) = \phi_z(x, y) .
\end{equation*}
}

\begin{lemma} \label{lem:stateful-hash}
    For all $Z \in \mathbb N$, there exists a linear transformation $\mathbf W$ such that,
    for all $x \in \mathbb R$ and $i \in \mathbb N$,
    \begin{equation*}
        \mathbf W \phi_z(x/i, 1/i) = \phi(x/i, 1/i) .
    \end{equation*}
\end{lemma}

\begin{proof}
    The subvector of $\phi_z(x/i, 1/i)$ from $4z + 1$ to $4(z + 1)$ is $\phi(x/i, 1/i)$. All other entries are zeros.
    We can recover $\phi$ from $\phi_z$ via a single linear transformation $\mathbf W$ that sums all elements of $\phi_z$ at offsets of $4$ to create a new vector of length $4$. 
\end{proof}

It also holds that the inner product over $\phi_z$'s, for fixed $z$, is equal to the inner product over $\phi$'s.
\ashish{for concreteness, would be better to extend \Cref{lem:stateful-hash} to also include the transformation that recovers $z$.}
Similarly to \Cref{lem:stateful-hash}, the state $z \in [0, Z]$ can be reconstructed from $\phi_z$ via a linear transformation that checks which entries are nonzero. The residual connection (before application of $\lnorm$) will similarly encode $z$.

\subsection{Rightmost Hard Attention with Layer-Norm Hash} \label{sec:rightmost-lnorm-hash}

% Here is a rough sketch of the ratio based reasoning I am thinking of:

% \begin{enumerate}
    % \item As before, let $\phi_x = \phi(x, 1)$, but let's only consider $x \in \R^+$, no negatives. Then, the information content of $\phi(x, y)$ is basically the same as that of the ratio $x/y$. (Insisting on no negatives as $\phi(-x, -y)$ would behave differently as a hash but would have the same ratio.)

    % \item Lemma Z: ... max is $\geq q$.

    % \item (DONE) Lemma A ($y''$ and $y'$ are on the \emph{same side} of $y$): Let $x, y, y', y'' \in \R^+$. If $y'' < y' \leq y$ or $y'' > y' \geq y$, then $\phi(x, y) \cdot \phi(x, y') > \phi(x, y) \cdot \phi(x, y'')$.

    % ALTERNATIVE: For $x, y, z \in \R+^$ and $z \geq y$, $\phi(x, y) \cdot \phi(x, z)$ is a decreasing function of $z - y$.
    
    % NOT TRUE: $\phi(x, y) \cdot \phi(x, z)$ is an increasing function of $|y - z|$.

    % \item Lemma B ($y''$ and $y'$ are on \emph{different sides} of $y$, ONLY one direction): Let $x, y, y', y'' \in \R^+$. If $y'' < y \leq y'$ and $y - y'' > y' - y$, then $\phi(x, y) \cdot \phi(x, y') > \phi(x, y) \cdot \phi(x, y'')$.

    % \item Lemma C: For any decreasing function $c_j$ of $j$, the conditions of Lemma A are satisfied for $x = q, y = c_i, y' = c_j, y'' = c_{\tilde{j}}$ for any $\tilde j < j \leq i$.  This means that among the $q$'s that are matched, the dot product will be the highest for the rightmost match.

    % \item Lemma D (rough, to be verified): For any \emph{sufficiently small (or some other adjective)} decreasing function $c_j$ of $j$ such as $c_j = 3j / (3j - 1)$, the conditions of Lemma B are satisfied for $x = q, y = c_i, y' = c_j, y'' = c_j x / x'$ for any $j < i$ and $x' \geq x + 1$. That is, $\phi(q, c_i) \cdot \phi(q, c_j) > \phi(x, c_i) \cdot \phi(x', c_j)$, where the last term follows from the invariant that $\phi(x', c_j) = \phi(x, c_j x / x')$. 

    % \item Lemma E: for $j \geq i/2$, $\ell \geq 1$, and $c_j = mj / (mj-1)$ for any $m > 2$
    % %, the best case for $q+\ell$ has a worse match to $(q, i)$ than the worst case for $q$ (which occurs for the smallest $j$, i.e., $i/2$).
    % $$
    % \max_{i/2 \leq j < i} \phi(q, c_i) \cdot \phi(q+\ell, c_j)
    %     <
    %     \min_{i/2 \leq j < i} \phi(q, c_i) \cdot \phi(q, c_j)
    % $$
    % \will{wlog prove for $q + 1$}
    % To this end, we show that with $c_j = mj / (mj-1)$ and any $m > 2$ (??), the best case for $q+1$ is in fact $(q+1, i/2)$, and that it is worse than $(q, i/2)$. Also note that in this case, $q+\delta$ will always be worse than $q+1$ for any $j$ and any $\delta > 1$.
% \end{enumerate}

\begin{proposition}
    \label{prop:theta}
    Let $x, y, w, z \in \Rpos$. Let $\theta$ denote the angle between the two 2-dimensional vectors $\langle x, y \rangle$ and $\langle w, z \rangle$ in $\R^2$. Then $\phi(x, y) \cdot \phi(w, z) = \cos(\theta)$.
\end{proposition}

\begin{proof}
    By the definition of $\phi$, we have:
    \begin{align*}
        \phi(x, y) \cdot \phi(w, z)
          & = \frac{\langle x, y, -x, -y \rangle}{\sqrt{2(x^2 + y^2)}} \cdot \frac{\langle w, z, -w, -z \rangle}{\sqrt{2(w^2 + z^2)}} \\
          & = \frac{2xw + 2yz}{\sqrt{2(x^2 + y^2)} \sqrt{2(w^2 + z^2)}} \\
          & = \frac{xw + yz}{\sqrt{x^2 + y^2} \sqrt{w^2 + z^2}} \\
          & = \frac{\langle x, y \rangle \cdot \langle w, z \rangle}{|| \langle x, y \rangle || \, || \langle w, z \rangle ||}
    \end{align*}
    This last quantity, by the geometric definition of dot product in Euclidean spaces, is $\cos(\theta)$.
\end{proof}

\begin{proposition}
    \label{prop:dot-product-monotone}
    Let $x, y, z \in \Rpos$. Then:
    % If $z \geq y$ (or $z \leq y$), then $\phi(x, y) \cdot \phi(x, z)$ is a decreasing (increasing, resp.) function of $z$ and is $1$ if and only if $z = y$.
    \begin{equation*}
        \phi(x, y) \cdot \phi(x, z) =
        \begin{cases*}
            1 & \text{if\ } $z = y$ \\
            \text{a decreasing function of\ } z & if $z \geq y$ \\
            \text{a increasing function of\ } z & if $z \leq y$
        \end{cases*}
    \end{equation*}
\end{proposition}

\begin{proof}
    By \Cref{prop:theta}, the dot product $\phi(x, y) \cdot \phi(x, z)$ is simply $\cos(\theta)$ where $\theta$ is the angle between the 2-dimensional vectors $\langle x, y \rangle$ and $\langle x, z \rangle$. Since both vectors have the same first dimension (namely, $x$), $\theta = 0$ (and hence $\cos(\theta) = 1$) precisely when $z = y$. Further, since $x, y, z$ are non-negative, $\theta$ increases as $z$ grows beyond $y$, which in turn decreases $\cos(\theta)$. It follows that, when $z \geq y$, the dot product is a decreasing function of $z$. The case where $z \leq y$ can be proved analogously.
\end{proof}

\begin{proposition} \label{prop:max}
    Let $q \in \mathbb N, k \in \Rplus,$ and $c_i, c_j \in \Rpos$.
    % with $c_j \neq 0$.
    Then $\phi(q, c_i) \cdot \phi(k, c_j)$
    has a unique local maximum w.r.t.~$k$ at $k = \frac{c_j}{c_i} q$.
\end{proposition}
\begin{proof}
    The squared inner product can be expanded as
    \begin{equation*}
        \frac{(qk + c_i c_j)^2}{(q^2 + c_i^2)(k^2 + c_j^2)} .
    \end{equation*}
    We now maximize this with respect to $k$ by taking the derivative, ignoring the $q^2 + c_i^2$ factor that does not depend on $k$:
    \begin{equation*}
        \frac{\partial}{\partial k} \left( \frac{(qk + c_i c_j)^2}{k^2 + c_j^2} \right) = \frac{2 c_j (c_j q - c_i k) (c_i c_j + kq)}{(k^2 + c_j^2)^2} .
    \end{equation*}
    % With $c_j \neq 0$ and $k \geq 0$,
    Given the ranges of $q, k, c_i,$ and $c_j$,
    the only root of this corresponds to
    \begin{align*}
        c_j q - c_i k &= 0 \\
        \implies k &= \frac{c_j}{c_i} q . \qedhere
    \end{align*}
\end{proof}

Having established these basic facts about the layer-norm hash, we will prove that the layer-norm hash can be used for a kind of ``rightmost'' hard attention \citep{hao2022ac0}: given a query $q$ at step $i$ and previous keys $k_1, \ldots, k_{i-1}$, we would like to attend to the \emph{largest} $j$ such that $k_j = q$. We will show that, if $c_i$ is set properly, this is possible. \Cref{lem:at-least-q} and \Cref{lem:q-plus-one-is-worse} establish that $j$ with the maximum attention score will satisfy $k_j = q$. \Cref{lem:q-most-recent} then shows that larger values of $j$ will receive more attention. This implies that the largest $j$ satisfying $k_j = q$ will be retrieved, as stated in \Cref{lem:rightmost-lnorm}.

\begin{lemma} \label{lem:at-least-q}
    Let $q \in \mathbb N$ and $c_i, c_j \in \Rpos$.
    % with $c_j \neq 0$.
    Then,
    \begin{equation*}
        \argmax_{k \in \mathbb N} \big\{ \phi(q, c_i) \cdot \phi(k, c_j) \big\} \geq q .
    \end{equation*}
\end{lemma}

\begin{proof}
    By \Cref{prop:max}, for any $q, i, j$, the only real-valued local maximum of $\phi(q, c_i) \cdot \phi(k, c_j)$ w.r.t.~$k$ is when $k = k^* \triangleq (c_j/c_i) q$. 
    Thus, the maximizer over $\mathbb N$ is at least  $\lfloor k^* \rfloor$
    % \ashish{changed a bit, to account for the case when $k^*$ is an integer}.
    % the greatest integer less than $k^*$.
    Since $c_i$ is decreasing with $i$ and  $j < i$, it follows that $1 \leq c_j / c_i$. Thus, $q \leq k^*$. Since $q \in \mathbb N$, we have $q \leq \lfloor k^* \rfloor$. It follows that the maximizer over $\mathbb N$ is at least $q$.
\end{proof}

\begin{lemma}
    \label{lem:q-plus-one-is-worse}
    Let $\ell, i, j, q \in \mathbb{N}, \epsilon \in \Rpos,$ and $m \in \Rplus$. Let $\ell \geq 1, i \geq 4, q \leq i, i/2 \leq j < i, \eps \leq 1/3,$ and $c_j = j / (j - \epsilon)$. Then %\{\lceil i/2 \rceil, \ldots i-1\}$,
    \begin{align}
        \label{eq:q-plus-one-is-worse}
        \max_j \big\{ \phi(q, c_i) \cdot \phi(q+\ell, c_j) \big\}
        & \, < \, \min_j \big\{ \phi(q, c_i) \cdot \phi(q, c_j) \big\}.
    \end{align}
\end{lemma}

\begin{proof}
    For simplicity, let $i_{\min} \triangleq \lceil i/2 \rceil$. We first consider the right hand side of inequality (\ref{eq:q-plus-one-is-worse}) in the statement of the lemma. Since $c_j$ is a decreasing function of $j$, we can apply \Cref{lem:q-most-recent} to conclude that the dot product $\phi(q, c_i) \cdot \phi(q, c_j)$ is an increasing function of $j$. It is therefore minimized when $j$ takes the lowest allowed value, namely $i_{\min}$. Thus, the right hand side of inequality (\ref{eq:q-plus-one-is-worse}) is simply $\phi(q, c_i) \cdot \phi(q, c_{i_{\min}})$.

    Now consider the left hand side. By the scale-invariance of $\phi$, we can rewrite $\phi(q+\ell, c_j)$ as $\phi(q, c_j \frac{q}{q+\ell})$. We will first show that $c_j \frac{q}{q+\ell} < c_i$. To this end, we have:
    \[
        c_j \frac{q}{q+\ell}
          \leq c_j \frac{q}{q+1}
          \leq c_j \frac{i}{i+1}
          \leq c_{i_{\min}} \frac{i}{i+1}
          = \frac{i_{\min}}{i_{\min}-\epsilon} \, \frac{i}{i+1}
          \leq \frac{i/2}{i/2-\epsilon} \, \frac{i}{i+1}
    \]
    Since $\epsilon < 1/2$, it can be verified that this last quantity is strictly smaller than $c_i = i / (i - \epsilon)$ whenever $i \geq 2$ \ashish{is there a simple proof of this??}. We can now apply \Cref{prop:dot-product-monotone} with $x = q, y = c_i,$ and $z = c_j$ and use the $z \leq y$ case to conclude that the dot product $\phi(q, c_i) \cdot \phi(q, c_j \frac{q}{q+\ell})$ is an \emph{increasing} function of $c_j \frac{q}{q+\ell}$, and hence an increasing function of $c_j$. Since $c_j$ is a decreasing function of $j$, the maximum in the left hand side of inequality (\ref{eq:q-plus-one-is-worse}) is achieved when $j$ has the smallest allowed value, $i_{\min}$. In other words, the left hand side of inequality (\ref{eq:q-plus-one-is-worse}) is simply $\phi(q, c_i) \cdot \phi(q, c_{i_{\min}} \frac{q}{q+\ell})$.

    At this point, proving the lemma reduces to showing that
    \begin{align}
        \label{eq:dot-product-at-imin}
        \phi(q, c_i) \cdot \phi(q, c_{i_{\min}} \frac{q}{q+\ell})
          & < \phi(q, c_i) \cdot \phi(q, c_{i_{\min}})
    \end{align}
    Note that $c_{i_{\min}} \frac{q}{q+\ell} < c_i < c_{i_{\min}}$, so we cannot directly use the monotonicity property from \Cref{prop:dot-product-monotone}. Instead, we will show that
    \begin{align}
        \label{eq:c_imin-is-closer}
        c_i - c_{i_{\min}} \frac{q}{q+\ell}
          & \geq c_{i_{\min}} - c_i
    \end{align}
    and argue that this is sufficient to prove inequality (\ref{eq:dot-product-at-imin}).

    First, in order to show that inequality (\ref{eq:c_imin-is-closer}) holds, we rewrite it as
    $2 c_i > c_{i_{\min}} \left(1 + \frac{q}{q+\ell}\right)$ and observe that it's sufficient to prove this for the smallest value of $\ell$, namely $1$. In other words, it suffices to have $c_i > c_{i_{\min}} \left( \frac{2q + 1}{2q + 2} \right)$. Since $\frac{2q + 1}{2q + 2}$ is an increasing function of $q$, it suffices to prove the inequality for the largest value of $q$, namely $i$. Additionally, $c_i = \frac{i}{i-\epsilon}$ and $c_{i_{\min}} = \frac{i_{\min}}{i_{\min}-\epsilon} \leq \frac{i/2}{i/2-\epsilon}$. It thus suffices to show:
    \begin{align*}
        \frac{i}{i-\epsilon} & > \frac{i/2}{i/2-\epsilon} \, \frac{2i+1}{2i+2} \\
        (i - 2\epsilon) (2i + 2) & > (i - \epsilon) (2i + 1) \\
        2i^2 + i (2 - 4\epsilon) - 4\epsilon & > 2i^2 + i (1 - 2\epsilon) - \epsilon \\
        i (1 - 2\epsilon) & > 3\epsilon
    \end{align*}
    which can be rewritten as $i > \frac{3\epsilon}{1 - 2\epsilon}$. Since $\epsilon \leq 1/3$, the right hand side is at most 3, while the left hand size, by a precondition of the lemma, is at least $4$.

    Second, to show that inequality (\ref{eq:c_imin-is-closer}) implies inequality (\ref{eq:dot-product-at-imin}), we again leverage the geometric interpretation of dot product in two dimensions and the fact that $\cos(\theta)$ is a decreasing function of $\theta$ for $\theta \in [0, \pi/2]$. By \Cref{prop:theta}, it suffices to show that the angle $\theta_{q+1}$ between the 2-dimensional vectors $\langle q, c_i \rangle$ and $\langle q, c_{i_{\min}} \frac{q}{q+\ell} \rangle$ is \emph{larger} than the angle $\theta_q$ between $\langle q, c_i \rangle$ and $\langle q, c_{i_{\min}} \rangle$. That is, $\theta_{q+1} > \theta_q$. Let $\delta \triangleq c_{i_{\min}} - c_i$. Consider the vector $\langle q, c_i - \delta \rangle$ and let $\theta_\delta$ be the angle between this vector and $\langle q, c_i \rangle$. By design, $\theta_\delta \leq \theta_{q+1}$. It therefore suffices to show that $\theta_\delta > \theta_q$, which we can rewrite as
    \begin{align*}
        \arctan\big(\frac{c_i}{q}\big) - \arctan\big(\frac{c_i - \delta}{q}\big)
          & \, > \, \arctan\big(\frac{c_i + \delta}{q}\big) - \arctan\big(\frac{c_i}{q}\big)
    \end{align*}
    That this inequality holds follows immediately from three facts: (a) the two arguments of $\arctan$ on both sides are equally far apart (specifically, $\delta/q$ apart); (b) the arguments on the left are smaller than the corresponding arguments on the right; and (c) the $\arctan$ function is increasing and \emph{concave} (i.e., has a decreasing derivative) in the range under consideration. This concludes the proof that inequality (\ref{eq:c_imin-is-closer}) implies inequality (\ref{eq:dot-product-at-imin}).
    
    We have shown that inequality (\ref{eq:dot-product-at-imin}) holds, and therefore the lemma holds.
    % ORIGINAL NOTES: \will{wlog prove for $q + 1$}
    % To this end, we show that with $c_j = mj / (mj-1)$ and any $m > 2$ (??), the best case for $q+1$ is in fact $(q+1, i/2)$, and that it is worse than $(q, i/2)$. Also note that in this case, $q+\delta$ will always be worse than $q+1$ for any $j$ and any $\delta > 1$.
\end{proof}

\begin{lemma}
    \label{lem:q-most-recent}
    For $q, i, j \in \mathbb{N}$ with $j \leq i$ and any decreasing function $c_j$ of $j$, $\phi(q, c_i) \cdot \phi(q, c_j)$ is an increasing function of $j$.
\end{lemma}

\begin{proof}
    By construction, $c_j \geq c_i$. Applying \Cref{prop:dot-product-monotone} with $x = q, y = c_i,$ and $z = c_j$ and using the $z \geq y$ case, it follows that the dot product $\phi(q, c_i) \cdot \phi(q, c_j)$ is a \emph{decreasing} function of $c_j$. Since $c_j$ itself is a decreasing function of $j$, the dot product is an increasing function of $j$.
\end{proof}

Combining all of the previous lemmas, we can obtain the main lemma used by the general Turing machine construction:

\begin{lemma}[Main Lemma] \label{lem:rightmost-lnorm}
    Let $q, k_1, \ldots k_{i-1} \in \mathbb{N}$
    and \will{preconditions}. Then $\phi(q, c_i) \cdot \phi(k_j, c_j)$ is maximized w.r.t.~$j$
    at the greatest $j < i$ such that $k_j = q$.
\end{lemma}

\begin{proof}
    TODO
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%

==> old/counter-automata.tex <==
The idea for simulating finite automata can be extended to simulate more general counter automata \citep{minsky1961recursive,fischer1966turing,merrill2021linguistic}. Counter automata are finite automata extended with integer-valued counter registers, which can be incremented, and decremented, and used to inform output and state transitions. We defer a formal definition and proof the following to \Cref{app:counter-automata}:

\begin{theorem}
    A transformer decoder with $t(n)$ CoT steps can simulate the state sequence of a $k$-counter machine for $t(n)$ steps.
\end{theorem}

Because a $k$-counter machine can simulate a Turing machine with doubly exponential time overhead \citep[][Theorem 1]{minsky1961recursive}, we get that a transformer with a very large number of steps can simulate a Turing machine:

\begin{corollary} \label{thm:counter-automata}
    A transformer with chain of thought can simulate a Turing machine with doubly exponential blowup in the number of steps:
    \begin{equation*}
        \TIME(\log \log t(n)) \subseteq \CoT(t(n)) .
    \end{equation*}
\end{corollary}

% APPENDIX BELOW

\section{Counter Automata} \label{app:counter-automata}

In this section, we extend the simulation construction for finite automata to show how a transformer with CoT can simulate a $k$-counter machine \citep{fischer1966turing}. Classically, for $k > 1$, the $k$-counter machine is Turing-complete, though it may take doubly exponentially long to simulate a Turing machine compared to the original run time \citep[][Theorem 1]{minsky1961recursive}.

A $k$-counter machine is a finite-state machine extended with $k$ counter registers. Formally, it is a tuple $\langle \Sigma, b, Q, q_0, \delta, F, k \rangle$ where all entries have the same definition as for Turing machines, except:
\begin{compactenum}
    \item $\delta$ is now a function of the form:
    \begin{equation*}
        Q \times (\Sigma \cup \{b\}) \times \{0, 1\}^k \to Q \times \{{\pm}1, {+}0 \}^k .
    \end{equation*}
    The second element in the result represents a function $\mathbb Z \to \mathbb Z$ in the natural way. \will{We can probably also simulate ${\times}0$, which could be useful because it might provide exponential speed up in some cases (don't have to decrement integer counters)}
    \item $k$ is a fixed-size integer specifying the number of counter registers.
\end{compactenum}

We define computation with a $k$-counter machine on an input $\sigma \in \Sigma^*$ as follows. A configuration is a finite state $q_i$ along with a register vector $\mathbf c_i \in \mathbb Z^k$.
We start with the initial state $q_0$ and the register vector $\mathbf c_0 = \vec 0$. Let the function $z : \mathbb Z^k \to \{0, 1\}^k$ be the function that checks elementwise equality to $0$.
Let $\sigma[j]$ be the $j$th token of $\sigma$ if $1 \leq j \leq \abs{\sigma}$ and $b$ otherwise.
At each time step $i$, if $q_i \not\in F$, we recurrently update the configuration via:
\begin{align*}
    \langle q_{i+1}, u_i \rangle &= \delta(q_i, \sigma[c_{i,0}], z(\mathbf c_i)) \\
    \mathbf c_{i+1} &= u_i(\mathbf c_i) .
\end{align*}
If $q_i \in F$ at any point, we accept $\sigma$. We define the language of the machine as the set of strings that it accepts.

\begin{theorem}
    A causal transformer with $t(n)$ chain-of-thought steps can simulate the state sequence of a $k$-counter machine for $t(n)$ steps.
\end{theorem}

\begin{proof}
The key idea is to simulate one step of a counter machine with one step of a transformer. At each position $i$, we will output a token $\delta_i \in \Delta$ encoding the output of the transition function at that step. That is, $\delta_i$ can be identified with a tuple $\langle q_i, u_i \rangle \in Q \times \{ {\pm} 1, {+}0 \}^k$ encoding the current controller state and local counter update. We will prove by induction this is possible.

In the base case of $i=1$, the previous token is not in $\Delta$, so we simply use the initial state $q_0$ and take the counter register to be $\vec 0$, meaning $z(\mathbf c_0) = \vec 1$. We can then compute $\delta_1 = \delta(q_0, \sigma_0, \vec 1)$ with a feedforward network.

In the inductive case, we have by assumption that the sequence of generated chain-of-thought tokens is $\delta_1, \ldots, \delta_i$. Our goal is to compute and output $\delta_{i+1} = \delta(q_i, \sigma_i, z(\mathbf c_i))$, which first involves computing the three arguments to $\delta$:
\begin{enumerate}
    \item Obtain the current finite state $q_i$ from $\delta_i$ via simple projection.
    \item Next, we will obtain the current input symbol $\sigma_i$. We apply \will{lem} to get a representation $1/i$ at CoT step $i$ as well as at the $i$th input token. We can then use a layer-norm hash construction to retrieve $\sigma_i$.
    \item We can attend over this sequence uniformly where the values are $u_i$ (a simple projection of $\delta_i$). This head computes the current counter register value $\mathbf c_i / i$ because
    \begin{equation*}
        \mathbf c_i = \sum_{j=1}^i u_j(\mathbf c_i) .
    \end{equation*}
    We can can check $z(\mathbf c_i)$ (whether the counters are $0$) by checking whether the attention head output vector is $0$ at each element.
\end{enumerate}
At this point, we have the current finite state, current input token, and zeroness of the current counter registers, so we can compute and outputs $\delta_{i+1} = \delta(q_i, \sigma_i, z(\mathbf c_i))$.
\end{proof}

==> old/definitions.tex <==
\subsection{Random Access Turing Machines}

\will{Think we can now cut this part?}

Beyond the Turing machine, we also study the ability of a transformer to simulate computation with random-access to memory. To this end, we adapt the following definition of a random access Turing machine \citep{immerman2012descriptive}.\footnote{Note that this is different (and generally weaker) than conventional random-access machine \citep{cook1973time}.}

\will{\url{https://en.wikipedia.org/wiki/Random-access_Turing_machine}. This idea seems to be we can write a number to a pointer tape and then retrieve the token at that position}

==> old/intro.tex <==
First, as a generic result, we find that power of transformers with $t(n)$ decoding steps is sandwiched between Turing machines with $t(n)$ time and Turing machines with $t(n) + \log n$ time:
\begin{equation*}
    \TIME(t(n)) \subseteq \CoT(t(n)) \subseteq \SPACE(t(n) + \log n) .
\end{equation*}
\will{mention quadratic upper bound here too?}
This shows that CoT does not just enable transformers to solve dynamic programming \citep{feng2023revealing}, but also simulate a Turing machine up to a bounded number of steps. On the other hand, it also establishes limits on the power of transformers with CoT as a function of the number of decoding steps.

We then explore how these results apply for two specific classes of interest: transformers with a linear number of decoding steps and transformers with a logarithmic number of decoding steps.

Having a linear number of CoT steps adds power.
For example, transformers with an $\O(n)$ scratchpad can recognize all regular languages, whereas transformers without a scratchpad cannot.\footnote{The negative result holds conditionally assuming $\TC^0 \neq \NC^1$. This follows because the word problem for the $5$-permutation group $S_5$ is both regular and $\NC^1$-complete.}
Thus, a scratchpad is not just beneficial for guiding the transformer's reasoning, but actually provides additional computational power to the model.

On the other hand, transformers with a logarithmic number of decoding steps obey similar limitations to standard transformer decoders: that is, they are upper bounded within uniform $\TC^0$. Transformers with $\O(\log n)$ CoT steps cannot solve directed graph connectivity or linear equalities, like transformers without CoT. On the other hand, we are able to show that transformers with $\O(n)$ CoT steps cannot solve problems beyond the context-sensitive languages, but it is open whether they can solve directed graph connectivity or linear equalities.

\will{Should we connect this to RLHF here? One benefit of RL is that the reward from the final answer conditions on the intermediate generation, unlike in standard pretraining.}

\will{This might be an argument to frame everything in terms of intermediate generation instead of chain-of-thought, because that's more generally what we're talking about. Chain-of-thought is a way to use intermediate generation at inference time, and RLHF is a way to train in a model with intermediate generation.}

==> old/old-lnorm-hash.tex <==
\begin{definition}[Layer-norm hash]
    Given a key $k \in \mathbb R$, its layer-norm hash is
    \begin{equation*}
        \hash(k) = \lnorm(k, 1, -k, -1) .
    \end{equation*}
\end{definition}

If a transformer represents a quantity $k_i$ at each column $i$, then it can directly compute $\hash(k_i)$ at each column. The useful thing about the layer-norm hash is that it will allow us to attend from column $i$ to another column $j$ where $k_i = k_j$. This follows from the following lemma if we pick an attention head that uses $\hash$ as queries and keys with a low temperature:

\begin{lemma} \label{lem:lnorm-hash}
    For two scalars $q, k$, $\hash(q) \cdot \hash(k)$ is maximized exactly when $q = k$.
\end{lemma}

\begin{proof}
    Let $\phi_k = \langle k, 1, -k, -1\rangle$ be the input vector to layer-norm.
    $\phi_k$ is constructed with mean $0$, so layer-norm reduces to $2$-normalization. Thus $\hash(k) = \phi_k / \norm{\phi_k}$, with $\norm{\phi_k} = \sqrt{2k^2 + 2}$.

    At this point, we turn to considering the inner product $\hash(q) \cdot \hash(k)$:
    \begin{align*}
        \hash(q) \cdot \hash(k)
        &= \frac{\phi_q}{\norm{\phi_q}} \cdot \frac{\phi_k}{\norm{\phi_k}} \\
        &= \frac{2qk + 2}{\sqrt{(2q^2 + 2)(2k^2 + 2)}} \\
        &= \frac{qk + 1}{\sqrt{(q^2 + 1)(k^2 + 1)}} .
    \end{align*}
    By definition, the inner product of unit-norm vectors is maximized at $1$.
    We show that, in fact, it achieves $1$ only when $q = k$, showing that that is the unique maximum:
    \begin{align*}
        1 &= \frac{qk + 1}{\sqrt{(q^2 + 1)(k^2 + 1)}} \\
        (qk + 1)^2 &= (q^2 + 1)(k^2 + 1) \\
        (qk)^2 + 2qk + 1 &= (qk)^2 + q^2 + k^2 + 1 \\
        2qk &= q^2 + k^2 \\
        0 &= (q - k)^2 .
    \end{align*}
    The original equation is only satisfied when $q = k$, so we conclude that $\hash(q) \cdot \hash(k)$ is maximized if and only if $q = k$.
\end{proof}

\subsection{Denominator-Invariant Layer-norm Hash}


==> old/perez-notes.tex <==
\section{Strange aspects of \citet{perez2021attention}}

\begin{enumerate}
    \item They use a somewhat nonstandard score function \emph{within} the attention mechanism rather than exp. Not a major issue
    \item Positional encodings include $i, 1/i, i/i^2$, which probably enables attending to target positions! 
    \item They are writing out $q, \sigma, m$, rather than computing $\sigma$ by summing over previous $m$'s. Probably not a fundamental difference, since they are basically just computing $\sigma$ one step early.
\end{enumerate}

==> old/tighter-log-steps.tex <==
\subsection{Circuit Upper Bound with Log Steps}

In fact, we can strength the characterization of $\CoT(\log n)$: we will show that it also falls in $\TC^0$. To get to the main result (\Cref{thm:tc0-upper-bound}), we first prove two key lemmas involving ``null padding'' of transformer decoders.

To, begin we define null-padded decoder transformers. This is a decoder-only transformer model where the token that gets added to the input buffer after each step is a special null character $\#$, not the token outputted by the previous step of the transformer.

Null-paddded transformers are relevant because normal transformer decoders can be simulated by them with an exponential blow up in the number of steps: 

\begin{lemma} \label{lem:poly-padding-tc0}
    For any polynomial $\poly$, a null-padded transformer decoder with at most $\poly(n)$ steps can be simulated in $\L$-uniform $\TC^0$.    
\end{lemma}

\begin{proof}
    The original $n$ steps of the transformer encoding the input can be computed in $\L$-uniform $\TC^0$ by \citet{merrill2023parallelism}.

    Each of the additional $t(n)$ decoding steps takes as input the position $i$ and, at each head, self-attends over the existing sequence of $n + i$ hidden states constructed at the previous layer.
    Without loss of generality, we show how to simulate one layer of one of these decoding steps.
    By the construction of \citet{merrill2023parallelism}, each attention head in the layer can be computed by an $\L$-uniform constant-depth $\TC^0$ circuit family.
    Analogously, their construction can be used to simulate the feedforward network on top of the head outputs.

    The whole network is then a finite-depth composition of these components, which can be stitched together analogously to \citet{merrill2023parallelism} in $\L$-uniform $\TC^0$.
\end{proof}

The analysis of standard transformers without additional decoding steps \citep{merrill2023parallelism} can be extended to show that such transformers are also in uniform $\TC^0$:

\begin{lemma} \label{lem:null-padding}
    A transformer decoder with $t(n)$ steps can be simulated by a null-padded transformer decoder with $\O(\exp(t(n)))$ steps and $1/i$ positional encodings.
\end{lemma}

\begin{proof}
    Assume we can enumerate all possible configurations of $c \log n$ tokens sequentially. Within each block of $c \log n$ tokens, we verify whether the original decoder transformer would have computed the $c \log n$ output tokens given the $n$ input tokens and $c \log n$ extra tokens. With one additional step at the end, we then retrieve the final output value from the block that corresponded to the correct output sequence of the original decoder only transformer.

    It remains to show that we can iterate all sequences of $c \log n$ tokens over $\Sigma$ in a null-padded transformer. We do this by using positional 

    \will{Running into issues here. how does this work if we cannot output?}
\end{proof}

At this point, we can state the main result:

\begin{theorem} \label{thm:tc0-upper-bound}
    A transformer decoder with at most $c \log n$ steps can only recognize languages in $\L$-uniform $\TC^0$.  
\end{theorem}

\begin{proof}
    Applying \Cref{lem:null-padding}, we see that a transformer decoder with $c \log n$ steps can be simulated by a null-padded transformer decoder with $\O(n^c)$ steps. By \Cref{lem:poly-padding-tc0}, such a transformer is in $\L$-uniform $\TC^0$. We conclude 
\end{proof}

From this result, we see that decoders with only a log number of steps obey the same limitations as transformers without any additional decoding steps. This is in contrast to a linear number of steps, where we saw that we were able to recognize all regular languages, which normal transformers cannot do. Thus, CoT will be unable to solve problems like graph connectivity or boolean formula evaluation unless more than a logarithmic number of decoding steps are allowed \citep{merrill2023parallelism}.

==> old/value-masked.tex <==
\subsection{Extending CoT Transformers' Power}

Finally, we propose the \textbf{value-masked transformer}: a minimal extension of the causally masked transformer that can simulate a Turing machine with CoT \emph{without} the exponential blowup incurred by standard transformers with CoT. The idea of the value-masked transformer is simple: we allow the transformer to optionally attend to a ``future'' key, in which case it retrieves the zero vector as a value. Doing this allows the transformer to compute uniform averages with comparable denominators at different positions in the sequence, which is crucial for our Turing machine simulation construction. We also describe a \textbf{layer-norm hash} construction that any transformer can use to attend to positions with exact-matching sums, which is especially useful for value-masked transformers because it enables retrieving based on exact match in uniform averages.

The value-masked transformer has better guarantees for expressive power, and we hypothesize that the construction underlying the Turing machine simulation could be generally useful for language processing. Empirically, we find that value-masked transformers can better learn to use a CoT compared to standard transformers, and also achieve stronger performance on standard language modeling benchmarks. We take this as evidence that value-masked attention is both theoretically and practically useful. \will{Best-case results :)}

\section{Value-Masked Transformers}

\will{This section is a bit out of place now because we don't have additional power. Maybe the framing could be: in theory, incomparable denominators are not an issue. But do they present an issue for learning? We introduce and test the value-masked transformer to find out.}

While we are able to simulate the state sequence for a Turing-complete $2$-counter machine with a standard transformer, we were not able to construct a simulation of a Turing machine state sequence directly. This implies that, while a transformer with chain-of-thought can simulate a Turing machine, it may need exponentially many more steps than the original Turing machine did (and these steps are already more expensive than simple Turing machine operations!).

In this section, we introduce the \emph{value-masked} transformer: a simple extension of the causally masked transformer that is able to directly simulate the state sequence of a Turing machine. The minimal extension of the transformer simply allows the transformer to attend ``into the future'' and retrieve the $\vec 0$ vector. At first glance, this may seem useless, but it has some powerful implications in the chain of thought setup: it allows the outputs of uniform heads at different time steps to be comparable, in the sense that they have the same denominator. This is important because it enables hard attention matching for equality in terms of the uniform head output.
This is perhaps a generally useful capability for chain-of-thought reasoning, but it is particularly useful in our context for being able to simulate a Turing machine tape correctly.

Formally, we define a value-masked transformer over $t$ steps as follows. In addition to the standard key $\mathbf k_i$, query $\mathbf q_i$, and value $\mathbf v_i$ at each time step $i$, we also compute a special ``future'' key $\mathbf k_i^*$. We then allow the transformer to put probability mass onto the future and retrieve $\vec 0$ with this key. Mathematically, this corresponds to simply redefining the normalizing constant in the attention computation as
\begin{align*}
    % \mathbf h_i &= \sum_{j \leq i} \frac{\exp(q_i^\top \cdot \mathbf k_j)}{Z_i} \mathbf v_j , \\
    Z_i &= \sum_{j \leq i} \exp(\mathbf q_i^\top \cdot \mathbf k_j) + (t - i) \exp(\mathbf q_i^\top \cdot \mathbf k_i^*) .
\end{align*}

To see how we will use this kind of attention, let $\mathbf k_j = \mathbf k_i^*$ for a fixed $i$ and all $j$. Then we recover a uniform sum over all $t$ timesteps, where the future timesteps ($j \geq i$) can be understood to have $\mathbf v_j = \vec 0$:
\begin{equation*}
    \mathbf h_i = \frac{1}{t} \sum_{j=1}^{t} \mathbf v_j .
\end{equation*}
In contrast, standard causally masked uniform attention can be recovered by setting $\mathbf k_j$ and $\mathbf k_i^* = 0$, yielding:
\begin{equation*}
    \mathbf h_i = \frac{1}{i} \sum_{j=1}^i \mathbf v_j .
\end{equation*}
Because the normalization depends on $i$, the head outputs are incomparable for different values of $i$. That is, we cannot straightforwardly compare $\mathbf h_i$ and $\mathbf h_j$ for $i \neq j$ and conclude whether the sums they capture are the same or not.

\subsection{Stronger Lower Bounds for Value-Masked Transformers}

We now show how value-masked attention and the layer-norm hash construction allow a transformer to simulate the state sequence of a Turing machine in real time.

\begin{theorem} \label{thm:lower-bound}
    A \will{value-masked} transformer with $t(n)$ chain-of-thought steps can simulate the state sequence of a Turing machine for $t(n)$ steps.
\end{theorem}

\begin{proof}
    The key idea is to simulate one step of a Turing machine run with one forward pass of the transformer. The main difficulty will be constructing a distributed representation of a Turing machine tape in a sequence of transformer state vectors and showing how the transformer can both maintain this representation and correctly reconstruct the current status of the tape at the head position. The key idea behind the construction will be to store ``diffs'' to the tape at each timestep, and then use attention to dynamically reconstruct the contents at the head position at every new timestep.

    % The Turing machine is captured by a transition function $\delta : Q \times \Sigma \to Q \times \Gamma \times \{\mathsf{L}, \mathsf{R}\}$.
    We introduce a new finite vocabulary $\Delta$ and identify each element of $Q \times \Gamma \times \{\pm 1 \}$ with some $\delta \in \Delta$. A deterministic Turing machine run of length $m$ induces a \emph{diff sequence} $\delta_0, \ldots, \delta_m \in \Delta$ capturing the state entered, token written, and direction moved after each token.
    The diff state sequence encodes all the information necessary to accept or reject a string with a Turing machine: simply project $\delta_i$ onto its first component $q_i$ and check whether $q_i \in F$.

    We show by induction over $i$ that we can construct a chain-of-thought transformer that outputs $\delta_i$ at step $i$.

    The first layer of the transformer, each position $i$ attends uniformly over the full context where the value at position $j$ is the third (move direction) component of $\delta_j$ at a CoT step and $0$ at other columns.\footnote{This can be easily extended to allow no-op moves.} The value of this head is thus $h_i/t(n)$, where $h_i$ is the position of the simulated TM head after $i$ steps.

    We can now apply a layer-norm hash to $j/t(n)$ in parallel at each $j < i$. By \Cref{lem:lnorm-hash}, we can hard-attend over these keys with query $h_i/t(n)$ to retrieve $\delta_{h_i}$, i.e., the last update written at position $h_i$.

    At this point, the transformer at position $i$ encodes $\delta_{h_i}$, whose second component is $\gamma_i$: the current contents of the cell at the head position. As input to this column of the transformer, we have $\delta_{i - 1}$, which encodes the current finite state $q_{i-1}$. We now compute $\delta_i = \delta(q_i, \gamma_i)$ using a feedforward network, which is possible because this computation is simply a finite table lookup. We write out $\delta_i$ as the output of the column.

    We conclude that we are able to simulate a Turing machine state sequence in real time with a value-masked transformer.
\end{proof}

The above result is tight (there is no constant factor on the number on the number of steps needed). This implies the following result in terms of time complexity classes:

\begin{corollary}
    Let $\CoT^*(t(n))$ denote the expressive power of the transformer with value-masked attention. Then,
    \begin{equation*}
        \TIME(t(n)) \subseteq \CoT^*(t(n)) .
    \end{equation*}
\end{corollary}

For example, this implies that a linear number of CoT steps can simulate deterministic pushdown automata, which is sufficient for capabilities like Dyck language recognition.

\section{Experiments with Value-Masked Attention}

Desired experiments:
\begin{enumerate}
    \item value-masked transformer vs. standard transformer on (natural) language modeling
    \item Train value-masked vs. standard transformer on x, CoT, y then evaluate accuracy when only x is given.
\end{enumerate}

\will{These experiments are most worth it if we do indeed think that value-masked attention adds power}
